Understanding Stay-at-home Attitudes through Framing Analysis of Tweets

With the onset of the COVID-19 pandemic, a number of public policy measures have been developed to curb the spread of the virus. However, little is known about the attitudes towards stay-at-home orders expressed on social media despite the fact that social media are central platforms for expressing and debating personal attitudes. To address this gap, we analyze the prevalence and framing of attitudes towards stay-at-home policies, as expressed on Twitter in the early months of the pandemic. We focus on three aspects of tweets: whether they contain an attitude towards stay-at-home measures, whether the attitude was for or against, and the moral justification for the attitude, if any. We collect and annotate a dataset of stay-at-home tweets and create classifiers that enable large-scale analysis of the relationship between moral frames and stay-at-home attitudes and their temporal evolution. Our findings suggest that frames of care are correlated with a supportive stance, whereas freedom and oppression signify an attitude against stay-at-home directives. There was widespread support for stay-at-home orders in the early weeks of lockdowns, followed by increased resistance toward the end of May and the beginning of June 2020. The resistance was associated with moral judgment that mapped to political divisions.

==> 4-classifiers-old.tex <==
\section{Classifying stay-at-home relevance, \\stance, and moral frame of tweets} 

We created classifiers for relevance, stance and moral frames of tweets using the annotated \emph{U.S. dataset} with the goal of automatically annotating and analyzing the much larger \emph{Global dataset}. 
We used 5-fold train/test splits on the \emph{U.S. dataset} for assessing the performance of each classifier and 5-fold cross validation on each training set for hyperparameter tuning. The best classifier was used for predicting the labels in the \emph{Global dataset}.

\subsection{Relevance classifier}
After removing the somewhat relevant tweets from the \emph{U.S. dataset}, we used it to remove the somewhat relevant tweets to train a new SVM relevance classifier. 
Similar to the initial relevance classifier described in the data section, we use the $word2vec$ embeddings as tweet features. The optimal specification for the SVM model with the new dataset is \{kernel='rbf',C=1 ,gamma=1\}. The model resulted in $78.7\%$ accuracy and $63\%$ precision. 
We trained a SVM classifier with the entire \emph{U.S. dataset} and best hyperparameters and then predicted stay-at-home relevant tweets in the \emph{Global dataset}. We obtained $206,333$ out of $5,538,993$ tweets as relevant. These relevant tweets have $914,909$ retweets.



\commentout{
\begin{table}[h]
\centering
\setlength{\tabcolsep}{5pt}
\begin{tabular}{|c|c|c|c|c|}\hline
Models &Precision&Recall&F-score  \\\hline
Random Forest&0.72&0.8&0.76\\
 Logistic Regression &0.69&0.76&0.73  \\
 Support Vector Machine&\textbf{0.89}&\textbf{0.95}&\textbf{0.92}\\
\hline
\end{tabular}
\caption{Relevance classifier performance.}
\label{table:relevance_classf}
\end{table}
}
\commentout{
\begin{table}[h]
\centering
\setlength{\tabcolsep}{5pt}
\begin{tabular}{|c|c|c|c|c|}\hline
Models &Precision&Recall&F-score  \\\hline
Random Forest&0.53&0.003&0.19\\
 Logistic Regression &0.57&0.27&0.37 \\
 Support Vector Machine&\textbf{0.63}&0.33&0.44\\
\hline
\end{tabular}
\caption{Relevance classifier performance.}
\label{table:relevance_classf}
\vspace{-10pt}
\end{table}
}

\commentout{
To characterize the tweets that signify stance towards stay-at-home (relevant tweets) vs. other stay-at-home tweets, we compare their predominant topics to the topics associated with irrelevant tweets using LDA~\cite{blei-jmlr} on the \emph{U.S. dataset}. Based on topic coherence we find the ideal number of topics to be 45 (with coherence value of 0.48). %
We rank these topics based on their frequencies of being the dominant topic in relevant tweets and irrelevant tweets. Table \ref{table:irr_rel_vocab} lists the 10 most frequent keywords in each of the top topics for relevant and irrelevant tweets. We observe that the most frequent topic for both relevant and irrelevant tweets are the same.} 
\commentout{
\begin{table}[h]
\centering
\caption{Top 10 keywords from the most frequent topics for irrelevant and relevant tweets.
}
\begin{tabular}{|c|c|c|}
 \hline
Topic&  Irrelevant & Relevant   \\ \hline
1    & \makecell{life, say, save,\\ american, point, virus,\\ deadly, voting,\\ protester, disease }& \makecell{life, say, save,\\ american, point,\\ virus, deadly, voting, \\protester, disease }  \\ \hline
2    & \makecell{lockdown, back, go, \\normal, friday, know,\\ vaccine, keep,\\ moron, sake }& \makecell{ care, family, protect,\\ live, health, must,\\ risk, free, dont, put}  \\ \hline
3    & \makecell{fuck, dont, stupid,\\ maybe, ignorant, turn,\\ jesus, totally,\\ twitter, sooner }& \makecell{ please, opening, dont,\\ definitely, forget,\\ post, old, crime,\\ truly, create}  \\ \hline
4    & \makecell{ still, protest, order,\\ number, go, pandemic,\\ believe, unless, \\understand, arizona}& \makecell{case, death, today,\\ rate, go, beach,\\ number, coronavirus,\\ county, hour }  \\ \hline
\end{tabular}
\label{table:irr_rel_vocab}
\vspace{-10pt}
\end{table}
}

\subsection{Tweet moral frame classifier}
\label{moral_frame_c}
To label the relevant tweets obtained from the relevance classifier, we used Snorkel \cite{snorkel}, a weakly supervised annotating method. Snorkel allows users to define labeling functions with heuristics based on a given task. It also supports the use of third-party models trained on related data as labeling functions. Snorkel provides a generative model that takes the output of labeling functions and either assigns a probabilistic label or abstains from labeling a data point. For this task we defined $13$ labeling functions. The first $12$ labeling functions labels a data point with one of the $12$ moral frames if a keyword for a frame from the MFT dictionary~\cite{Graham2013} is present in a tweet. The last labeling function is based on a classifier trained on \emph{U.S. dataset} having $2,400$ annotated phrases.

Since the dataset is small in size and has class imbalance, we made some modifications. In each training fold of the five fold  cross-evaluation, %
we under-sampled tweets having the \textit{Care} moral frame to $500$ (since the dataset is skewed towards \textit{Care}).Then we added tweets from the MFTC dataset\cite{dehghani} for the remaining moral frames \textit{Harm, Fairness, Injustice, Loyalty, Betrayal, Purity, Degradation, Authority and Subversion} to make the count of tweets 500 for each of these frames. The MFTC dataset \cite{dehghani} does not have samples for the remaining two frames - \textit{Freedom and Oppression}, so we oversampled these two moral frames with the ADASYN~\cite{adasyn} python library.     %



Using this modified training data, we trained three models - a \textit{Support Vector Machine Classifier}(with optimum hyperparameters \{C = 10, gamma = 0.01, kernel = rbf\}, a \textit{Random Forest Classifier} (the best hyperparameters being \{n\_estimators = 100, criterion = entropy\} and a
\textit{BiLSTM} classifier. The first two classifiers are built using scikit-learn python library.The \textit{BiLSTM} classifier is implemented with Keras python library and has an Embedding layer, a Bidirectional LSTM layer  and a 12 unit dense layer. The model performs best with 120 hidden units in the  Bidirectional LSTM layer, softmax activation, categorical cross-entropy loss function and Adam optimizer. This model is trained for 50 epochs with early stopping. With this classifier, 100d GloVe \cite{pennington-etal-2014-glove} embeddings (trained on Twitter data) are used to represent each word in the vocabulary.
We also explore three baselines for this task. We build a
 a \textbf{Keywords classifier} where tweets are labeled with a moral frame if they contain a keyword from the MFT dictionary~\cite{Graham2013} and check if the labels match with the ground truth. In case there is a match with keywords from more than one moral frame, during evaluation if one of them is same as the ground truth, it is considered to be a true positive. 
The other baseline is a \emph{Random Forest Classifier} trained on Moral Foundations Twitter Corpus(MFTC) \cite{dehghani} and evaluated on our test dataset. %
The best model has hyperparameters \{n\_estimators = 100, criterion = entropy\} and this is used for evaluation of the test dataset. Finally we build a random classifier where we randomly assign classes to the tweets in the dataset.

The results obtained from the baselines and our models on this classification task are reported in Table \ref{table:moralframe_classf} where the macro and weighted F-scores obtained are listed.
The \textit{BiLSTM + GloVe} model is found to be the best classifier. We use the hyperparameters for this classifier and train a new \textit{BiLSTM + GloVe} model on the entire dataset of $2,400$ tweets along with the modifications mentioned above. Then we use this model as one of the labeling functions for the Snorkel framework.

Snorkel labels $65\%$ of the $206,333$ relevant tweets with one of the $12$ moral frames and the rest $35\%$ it abstains from labeling. To label these $35\%$ tweets, we use the \textit{BiLSTM + GloVe} classifier, the one used as a labeling function in the Snorkel framework. The final distribution of predicted moral frames is shown in Table~\ref{table:mf-stance}. 



\begin{table}[h]
\centering
\caption{Moral Frame Classification.}
\setlength{\tabcolsep}{5pt}
\begin{tabular}{|c|c|}\hline
Models & \makecell{Macro/Weighted\\ F-score} \\\hline
 Random Classifier & 0.05/0.09 \\
 Random Forest Classifier (MFTC) & 0.09/0.28\\
 Keywords Classifier & 0.15/0.34 \\
 Support Vector Machine Classifier  & 0.15/0.39 \\
 Random Forest Classifier & 0.17/0.40 \\
 BiLSTM + GloVe  & \textbf{0.41/0.64}\\
\hline
\end{tabular}
\label{table:moralframe_classf}
\vspace{-12pt}
\end{table}

\subsection{Tweet stance classifier}
We use the $1,779$ tweets for stance classification because all phrases within any given tweet have the same stance. In each fold of five fold cross validation, a stratified 80-20 split of the data is performed. Oversampling is done on the training dataset using ADASYN \cite{adasyn} python library. We train three classifiers on this training dataset - \textit{Support Vector Machine Classifier} (performs best with hyperparameters \{C = 10, gamma = 0.01, kernel = rbf\}), 
\textit{Random Forest Classifier} (where the optimum hyperparameters are \{criterion = entropy, n\_estimators = 100\}) and a \textit{BiLSTM} classifier.
We implement the setup for \textit{BiLSTM} classifier with functions from Keras python library.It has an Embedding layer, a Bidirectional LSTM layer and a 3 unit dense layer. To represent words in the vocabulary, 100d GloVe \cite{pennington-etal-2014-glove} word embeddings trained on Twitter data are used in this classifier.The best hyperparameters for the model have 128 hidden units and a dropout of 0.2 in the Bidirectional LSTM layer, softmax activation, categorical cross-entropy loss function and Adam optimizer. The model is trained for 50 epochs with early stopping. %


\begin{table}[h]
\centering
\caption{Stance Classification.}
\begin{tabular}{|c|c|}\hline
Models &  \makecell{Macro/Weighted\\ F-score} \\\hline
 Random Classifier & 0.23/0.43 \\
 Support Vector Machine Classifier & 0.30/0.75 \\
 Random Forest Classifier  & 0.37/0.75 \\
 BiLSTM + GloVe  & \textbf{0.46/0.78} \\
 
\hline
\end{tabular}
\label{table:stance_classf}
\vspace{-5pt}
\end{table}

Table \ref{table:stance_classf} shows the performance of the classifiers for this task. The macro and weighted F-scores obtained for all the models are reported and the \textit{BiLSTM + GloVe} classifier outperforms the other models.
Using the hyperparameters of the best model, we train a new \textit{BiLSTM + GloVe} classifier on the entire \emph{U.S. dataset} and use that to predict labels for the $206,333$ relevant tweets. %
The distribution of stance of the tweets obtained after the prediction is  \{\textit{For}: $142,780$; \textit{Against}: $52,740$; \textit{Undecided}: $10,813$\}.






















\commentout{

\begin{enumerate}
    \item Relevance
    \begin{itemize}
        \item Relevant: Tweets clearly expressing an attitude related to Stay at Home.
        \item Somewhat  Relevant: Tweets that are tangentially related to Stay at Home and/or the attitude expression can be inferred but is not clearly stated.
        \item Irrelevant: Tweets not related to Stay at Home.
    \end{itemize}
    
    \item Attitude
    \begin{itemize}
        \item Pro: Relevant tweets with attitudes in support of Stay at Home.
        \item Con: Relevant tweets with attitudes in opposition of Stay at Home or in support of reopening.
    \end{itemize}
    
    \item Tweet Quality: Coded only if tweets are coded as Relevant and express a Pro or Con attitude.
    \begin{itemize}
        \item Vivid: Tweets that use a specific example involving a personal relationship or experience.
	\item Generic: Tweets that use general examples or broad statistics. 
    \end{itemize}
    
    \item Moral Foundation: Coded only if tweets were coded as Relevant and have a Pro or Con attitude. \fixme{zf: We used the moral foundation dictionary created by Graham et al. \cite{graham-jpsp09}. The dictionary contains the words and word stems associated with ten moral frames. We added two additional frames based on Liberty, a candidate MFT frame. }
    \begin{itemize}
        \item Care: Attitudes based on the need to help or protect oneself or others.
\item Harm: Attitudes based on the fear of damage or destruction to oneself or others.
\item Fairness: Attitudes based on the need for justice or equality.
\item Injustice: Attitudes based on the fear of prejudice, inequality, or wrongdoing.
\item Loyalty: Attitudes based on the needs of the collective or group allegiance.
\item Betrayal: Attitudes based on the fear of unfaithfulness or acting against the needs of the collective.
\item Authority: Attitudes based on respect for authority figures or rules.
\item Subversion: Attitudes based on rebellion against authority figures or rules.
\item Purity: Attitudes based on piety or the fulfillment of religious obligations.
\item Degradation: Attitudes based on depravity or failure to fulfill religious obligations.
\item Liberty: Attitudes based on the need for freedom or constitutional rights.
\item Oppression: Attitudes based on the fear of tyranny, subjugation, or loss of constitutional rights.
    \end{itemize}

\end{enumerate}
}























\commentout{
\begin{table}
\centering
\setlength{\tabcolsep}{5pt}
\begin{tabular}{|l|r|r|r|r|}
\hline
Moral Frame & \multicolumn{3}{c|}{Stance} & Total  \\ \cline{2-4}
& Positive & Negative & Undecided & \\\hline
Care & 1049 & 16 & 10 & 1075 \\
Harm & 420 & 93 & 10 &  523 \\
Fairness & 17 & 1 & 1 & 19 \\
Injustice & 16 & 11 & 0 & 27 \\
Loyalty & 232 & 9 & 3 & 244 \\
Betrayal & 49 & 5 & 1 & 55 \\
Authority &  174 & 5 & 1 & 180\\
Subversion & 25 & 28 & 11 & 64\\
Purity & 40 & 3 & 0 & 43 \\
Degradation & 6 & 1 & 0 & 7 \\
Freedom & 26 & 94 & 6 & 126 \\
Oppression & 4 &  60 & 0 & 64 \\


\hline
Total & 2058 & 326 & 43 & 2427\\
\hline
\end{tabular}
\caption{Distribution of moral frames by stance}
\label{table:mf-stance}
\end{table}
} %










 



\commentout{

\begin{figure}[h]
    \centering
        \includegraphics[width=0.5\textwidth]{fig/SAH.png}
        \caption{Nomenclature and formation of different data sets from initial main data set}
    \label{fig:Stay-at-Home Data Sets}
\end{figure}
}

\commentout{ 
 \begin{table}
\centering
\setlength{\tabcolsep}{5pt}
\begin{tabular}{|c|c|c|}
 \hline
Topic& Weight * Word   \\ \hline
1    & \makecell{0.088 * home; 0.049 * stay; 0.036 * corona;\\ 0.024 * virus; 0.023 * people; 0.021 * work;\\ 0.012 * love; 0.012 * stop; 0.012 * want;\\ 0.011 * stick}    \\ \hline
2    & \makecell{0.047 * quarantin; 0.038 * covid;\\ 0.038 * coronavirus; 0.031 * open;\\ 0.028 * stayhom; 0.027 * like; 0.017* thank;\\ 0.013* pandem; 0.013 * look}    \\ \hline
3    & \makecell{0.045 * home; 0.040 * time; 0.030 *stay;\\ 0.028 * distanc; 0.027 * social; 0.014 * covid;\\ 0.014 * life; 0.013 * miss}    \\ \hline
4    & \makecell{0.141 * home; 0.141 * stay; 0.044 * order;\\ 0.023 * peopl; 0.021 * work; 0.015 * need;\\ 0.012 * close;0.011 * open; 0.010 * essenti}    \\ \hline
\end{tabular}
\caption{The stay-at-home candidate keywords and their weights in each of four topics extracted by LDA model}
\label{table:lds_keywords}
\end{table}

}


\commentout{
One of our main goals in this paper is to assess the
attitude, sentiment and virality of tweets of users in USA. Hence, we filtered for tweets originated from USA. Using the 'place' attribute \cite{twitter_objects} we further filtered the data set with country\_code = US. The data set formed by such filtering is around 0.5\% of the original data set. We refer too this dataset as \textit{US-based dataset}. This dataset includes \fixme{0.5\% }of collected English tweets.

For our purposes of Natural Language processing, we needed to preprocess the text of tweets. First, we removed all the punctuation and HTML addresses. Then, the text were tokenized in order to convert sentences into words. The tokens were further stemmed to remove suffixes and prefixes and then lemmatized to get the original form of word to maintain consistency.

One of our main goals in this paper is to assess the
attitude, sentiment and virality of tweets of users in USA. Hence, we filtered for tweets originated from USA. Using the 'place' attribute \cite{twitter_objects} we further filtered the data set with $country\_code = US$. The data set formed by such filtering is around 0.5\% of the original data set. We refer too this dataset as \textit{US-based dataset}. This dataset includes \fixme{0.5\% }of collected English tweets.
\begin{figure*}[h]
     \centering
     \begin{subfigure}[h]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/type_dis.jpg}
         \caption{Distribution of tweets}
         \label{fig:y equals x}
     \end{subfigure}
     \begin{subfigure}[h]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{fig/language_dist.jpg}
         \caption{Distribution of tweets based on the languages}
         \label{fig:five over x}
     \end{subfigure}
        \caption{Distribution}
        \label{fig:three graphs}
\end{figure*}
\subsubsection{Detecting stay at home tweets}
In order to separate stay-at-home tweets from the rest, we considered two different approaches:
\begin{itemize}
    \item keyword\_based approach: In this method, we find stay-at-home tweets using the following steps:
    \begin{itemize}
\item Preprocessing: We created two corpus of the processed tweet texts using methods of Bag of Words and TFIDF. The corpus was stored with 100,000 words in form of dictionary with extremes removed, like words occurring less than 15 times. All the tweet texts were also transformed to lower case too.

\item Finding underlying topics: On both the corpus of Bag-of-words and TFIDF, we used latent Dirichlet allocation (LDA) \cite{blei-jmlr} to find the underlying topics of tweets. LDA gave us 20 topics in form of keywords associated with those topics and their weights. In order to find the topics related to stay-at-home, we created 10 tweets that contain different type of stay-at-home related text. These manually created tweets were classified into those 10 topics with a similarity score for each topic. We selected the cumulative top 4 topics and their keywords for further analysis.
\fixme{what are 10 and 4 here?}

\item Finding Stay-at-home keywords: From topics and their keywords generated by the LDA analysis, we picked keywords that can be termed as directly related to stay-at-home topic. Furthermore, we checked 100 tweets gained exclusively by each keyword.

\item Finalizing Keywords:  Using WordNet \cite{miller-princeton} we also discovered synonyms and relating words to the main keywords that were found. Moreover, we analyzed bi-grams and tri-grams \cite{chelba-arXiv} to find related keywords or sets of words. After checking all the tweets exclusively gained by keywords, we selected final keywords for filtering stay-at-home data set by string matching are Home, Open, Quarantine, Lockdown, Inside.
\end{itemize}

    \item Stay-at-home attitude classifier: Our definition for a tweet to be consisting of one or more stay-at-home attitude is:

“We define a tweet as relevant for our analysis of stay-at-home (SAH) attitudes if its content expresses support for or opposition to such public directives. The origins of such directives need not be local. They may also have been issued by authorities in places other than the message sender’s home location. They may also be responses to such directives by others, including political and media elites, as well as those whose attitudes or behaviors have become known to the sender. We regard the reporting of Stay-at-Home directives by message senders as tantamount to support. We also regard the use of two or more relevant hashtags alone as equivalent to an attitude on the assumption that such effort, even though unaccompanied by original content, is indicative of a genuine underlying opinion.”

\fixme{Vipul: Is is 5000 or ~7100? its around 7100 in SAH3 from march to june and the random sample given was of 1221 tweets}
Deriving a random representative sample of 5,000 tweets from stay-at-home data set gained by keyword matching from US based data set, we manually classified each tweet for having a stay-at-home attitude or for not having a stay-at-home attitude. The binary classification is done according to the definition stated above.

We converted the preprocessed tweet texts to vectors using Word2vec \cite{mikolov-acm} and averaged them to make a single vector for each tweet. The manually annotated data set is used for training  Support-Vector Machine (SVM) model. The optimum specifications for SVM model were \}kernel = 'rbf',C = 10 , gamma = 0.1\}. The model resulted in 88\% accuracy, with a well balanced confusion matrix. Total tweets with an attitude were 0.03\% of the main data set.
\end{itemize}

Using keyword\_based approach and Stay-at-home attitude classifier, we filtered English\_tweets dataset and extracted different datasets as following\fixme{mention the number of tweets in each dataset Vipul: "for march to june or july?"
for march to june, we have the numbers as - 
SAH0 = 13.68 million
SAH1 = 68,900
SAH2 = 32,456
SAH3 = 7121
SAH4 = 1.21 million
SAH5 = 7121}:
\begin{itemize}
\item SAH0 - Set filtered for Stay-at-home tweets using keyword matching
\item SAH1 - US-based dataset filtered for stay-at-home tweets using keyword matching
\item SAH2 - US-based dataset filtered for stay-at-home attitude tweets using Stay-at-home attitude classifier
\item SAH3 - SAH1  filtered for tweets with one or more Stay-at-home attitude using Stay-at-home attitude classifier
\item SAH4 - SAH0 filtered for tweets with one or more Stay-at-home attitude using Stay-at-home attitude classifier
\item SAH5 - SAH2 filtered by using keyword matching to confirm if it is almost similar to SAH3 or not. It was very similar.

The Flowchart 1 also explains the formation of different data sets.
\end{itemize}
\begin{figure}[h]
    \centering
        \includegraphics[width=0.5\textwidth]{fig/SAH.png}
        \caption{Nomenclature and formation of different data sets from initial main data set}
    \label{fig:Stay-at-Home Data Sets}
\end{figure}

\commentout{
\subsection{Frame Analysis}
\fixme{Describe moral frame stuff here.}
\subsubsection{Relevance Classifier}
We define a tweet to be \textit{Relevant} if it has at least one moral frame. Otherwise, it will be considered "Irrelevant".
\fixme{describe how we annotated phrases and tweets here}.  With the aim of finding relevant tweets, we annotated $7100$ tweets of $SAH3$ dataset manually and we found 1804 Relevant tweets. Using the ground truth, we build a Relevance Classifier that predict the relevancy of tweets. After preprocessing the tweets and conveting tweets to vectors using word2vec, we use SVM algorithm with 78\% accuracy on the subsampled dataset. Then we applied this classifier to predict the relevancy of SAH0, SAH1 and SAH4 datasets.
\fixme{how many tweets in each of them and the new name of them}

}
\commentout{
\subsection{Detecting stay-at-home tweets using keywords}
In order to separate stay-at-home tweets from the rest, we found stay-at-home related keywords using machine learning tools. In the preporcessing step, we split the text of tweets into sentences and the sentences into words, lowercased the words and removed punctuation. We removed stopwords, lemmatized the words and stemmed them. 
To tokenize the texts of tweets in the dataset, we applied TFIDF and Bag of Words methods separately on the data. Then, we used latent Dirichlet allocation (LDA) \cite{blei-jmlr} to find the underlying topics of tweets. 
LDA found 10 topics in the dataset in the form of keywords associated with those topics and their relative weights.

To find the most relevant topics to SAH,
 we created 10 SAH related sentences manually and detect the four most frequent topics from 10 topics in these sentences. We obtained \fixme{keywords from these topics}. \fixme{Then, we manually selected keywords that seemed more SAH relevant keywords for further analysis.} Using WordNet \cite{miller-princeton}, we found synonyms and relating words to the main keywords that we found in the previous steps. Moreover, we analyzed bi-grams and tri-grams \cite{chelba-arXiv} to find related keywords or set of words. For each keyword, we extracted tweets containing  just that keyword from Eng\_dataset and sampled  100 tweets of these tweets randomly. Then, we manually checked whether these tweets are SAH relevant or not. Keywords observed in
 at least 80 SAH relevant tweets, were considered as the final SAH keywords that are : Home, Open, Quarantine, Lockdown, Inside.
 Then, we filtered Eng\_dataset using these keywords and obtained \textbf{Main\_datase}.
 }
 \commentout{
In order to separate stay-at-home tweets from the rest, we considered the following steps:
\begin{itemize}
\item \textbf{Preprocessing}: We created two corpus of the processed tweet texts using methods of Bag of Words and TFIDF. The corpus was stored with 100,000 words in dictionary form with extremes removed, for example words occurring less than 15 times. All the tweet texts were also transformed to lower case.
\item \textbf{Finding underlying topics}: On both the corpus of Bag-of-words and TFIDF, we used latent Dirichlet allocation (LDA) \cite{blei-jmlr} to find the underlying topics. LDA gave us 10 topics in the form of keywords associated with those topics and their weights. In order to find the topics related to stay-at-home,
\fixme{check with Vipul:we created 10 tweets (Vipul: sentences?) that contain different type of stay-at-home related text.} These manually created tweets were classified into those 10 topics with a similarity score for each topic. We selected the cumulative top 4 topics and their keywords for further analysis.
\fixme{what are 10 and 4 here? Vipul: "10 SAH sentence to see which of the topics comes on the top and we choose top 4 overall".}
\item \textbf{Finding Stay-at-home keywords}: From topics and their keywords generated by the LDA analysis, we picked keywords that can be termed as directly related to stay-at-home topic. Furthermore, we checked 100 tweets gained exclusively by each keyword.
\item \textbf{Finalizing Keywords}: Using WordNet \cite{miller-princeton}, we found synonyms and relating words to the main keywords that we found in the previous steps. Moreover, we analyzed bi-grams and tri-grams \cite{chelba-arXiv} to find related keywords or set of words. After checking all the tweets exclusively gained by keywords, we selected final keywords for filtering stay-at-home dataset by string matching: Home, Open, Quarantine, Lockdown, Inside. We refer to this dataset as \textit{Keyword\_based dataset} which includes \fixme{$13 M$} English language tweets from March to June $2020$ from all over the world.
\end{itemize}
}


}

\commentout{
Domain experts on our team manually detected which of the $7,161$ tweets contain a stay-at-home attitude.
Each tweet might contain more than one phrase and some phrases may not be relevant. 
\fixme{zf ask Lauren: As long as at least one phrase of a tweet contained a stay-at-home attitude, we consider the tweet as relevant.
We convert tweets to phrases and conduct the annotation at the phrase level. }
We identified $2,400$ phrases as relevant, $4,734$ as irrelevant, and $27$ as somewhat relevant.}








\commentout{\begin{enumerate}
    \item Relevance
    \begin{itemize}
        \item Relevant: Tweets clearly expressing an attitude related to Stay at Home.
        \item Somewhat Relevant: Tweets that are tangentially related to Stay at Home and/or the attitude expression can be inferred but is not clearly stated.
        \item Irrelevant: Tweets that are not related to Stay at Home.
    \end{itemize}
    
    \item Attitude
    \begin{itemize}
        \item Pro: Relevant tweets with attitudes in support of Stay at Home.
        \item Con: Relevant tweets with attitudes in opposition of Stay at Home or in support of reopening.
    \end{itemize}
    
    \item Tweet Quality: Codeed TQ only if tweets are coded as Relevant and have a Pro or Con attitude.
    \begin{itemize}
        \item Vivid: Relevant tweets with a Pro or Con attitude that use a specific example involving a personal relationship or experience.
	\item Generic: Relevant tweets with a Pro or Con attitude that use general examples or broad statistics. 
    \end{itemize}
    
    \item Moral Foundation: Coded MF only if tweets are coded as Relevant and have a Pro or Con attitude. \fixme{We used moral foundation dictionary created by Graham et al. \cite{graham-jpsp09}. This dictionary includes the words and word stems associated with twelve moral frames.}
    \begin{itemize}
        \item Care: Attitudes for or against Stay at Home based on the need to help or protect oneself or others.
\item Harm: Attitudes for or against Stay at Home based on the fear of damage or destruction to oneself or others.
\item Fairness: Attitudes for or against Stay at Home based on the need for justice or equality.
\item Injustice: Attitudes for or against Stay at Home based on the fear of prejudice, inequality, or wrongdoing.
\item Loyalty: Attitudes for or against Stay at Home based on the needs of the collective or group allegiance.
\item Betrayal: Attitudes for or against Stay at Home based on the fear of unfaithfulness or acting against the needs of the collective.
\item Authority: Attitudes for or against Stay at Home based on respect for authority figures or rules.
\item Subversion: Attitudes for or against Stay at Home based on rebellion against authority figures or rules.
\item Purity: Attitudes for or against Stay at Home based on piety or the fulfillment of religious obligations.
\item Degradation: Attitudes for or against Stay at Home based on depravity or failure to fulfill religious obligations.
\item Liberty: Attitudes for or against Stay at Home based on the need for freedom or constitutional rights.
\item Oppression: Attitudes for or against Stay at Home based on the fear of tyranny, subjugation, or loss of constitutional rights.
    \end{itemize}

\end{enumerate}}

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************

